A Memory-Efficient Dynamic Image Reconstruction Method using Neural Fields

Dynamic imaging is essential for analyzing various biological systems and behaviors but faces two main challenges: data incompleteness and computational burden. For many imaging systems, high frame rates and short acquisition times require severe undersampling, which leads to data incompleteness. Multiple images may then be compatible with the data, thus requiring special techniques (regularization) to ensure the uniqueness of the reconstruction. Computational and memory requirements are particularly burdensome for three-dimensional dynamic imaging applications requiring high resolution in both space and time. Exploiting redundancies in the object's spatiotemporal features is key to addressing both challenges. This contribution investigates neural fields, or implicit neural representations, to model the sought-after dynamic object. Neural fields are a particular class of neural networks that represent the dynamic object as a continuous function of space and time, thus avoiding the burden of storing a full resolution image at each time frame. Neural field representation thus reduces the image reconstruction problem to estimating the network parameters via a nonlinear optimization problem (training). Once trained, the neural field can be evaluated at arbitrary locations in space and time, allowing for high-resolution rendering of the object. Key advantages of the proposed approach are that neural fields automatically learn and exploit redundancies in the sought-after object to both regularize the reconstruction and significantly reduce memory storage requirements. The feasibility of the proposed framework is illustrated with an application to dynamic image reconstruction from severely undersampled circular Radon transform data.

==> math_notations.tex <==
\section{Mathematical Notation}
Table \ref{tab:notation} summarizes the mathematical notations and symbols used in this work.


    \label{tab:notation}
\begin{table}[H]
    \centering
    \caption{Table of mathematical notations and symbols}
    \begin{tabular}{c|l}
        $\ipar \in \mathbb{U}$ & Infinite dimensional image  \\
        $\data \in \D$ & Finite dimensional measurements \\ 
        $\H:\mathbb{U} \rightarrow \D$ & Continuous-to-discrete imaging operator\\
        $\mathbf{H}:\R^{NK} \rightarrow \D$& Discrete-to-discrete imaging operator\\
        $\noise \in \D$ & Additive noise in measurement space \\ 
        $\sigma\in \R$ & Standard deviation of white Gaussian noise \\ 
        $x \in \Omega$ & Spatial coordinates for image \\ 
        $t \in [0,T]$ & Time coordinates for image\\
        $\Omega_T = \Omega \times [0,T]$ & Domain over which image coordinates are defined \\ 
        $\LI:\mathbb{U}\rightarrow \R$ & Continuous data fidelity functional \\
        $\mathbf{L}:\R^{NK} \rightarrow \R$& Discrete data fidelity function \\
        $\Reg: \mathbb{U}\rightarrow \R$ & Regularization functional \\ 
        $\mathbf{R}:\R^{NK} \rightarrow \R$& Discrete regularization function\\
        $\J = \LI + \Reg$ & Continuous cost functional\\
        $\mathbf{J} = \mathbf{L} + \mathbf{R}$& Discrete cost function\\
        $N$ & Number of pixels \\ 
        $K$ & Number of frames \\ 
        $\boldsymbol{\ipar } \in \R^{NK}$ & discrete representation of $\ipar$ \\
        $\{\beta_n:\Omega \rightarrow \R\}_{n=1}^N$ & basis for discrete representation. \\ 
        $\alpha \in \R^{K*N}$ & spanning coefficients for discrete representation \\ 
        $D_\nabla$ & finite difference gradient operator \\ 
        $TV_D$ & Discrete total variation using finite-differences\\
        $TV_S$ & Stochastic total variation using automatic differentiation \\ 
        $\boldsymbol{F} \in \R^{N \times K}$ & matrix representation of spanning coefficients \\ 
        $\operatorname{Nuc}:\R^{N\times K} \rightarrow \R$ & Nuclear norm functional\\
        $\gamma > 0$ & regularization weight\\ 
        $\xi \in \R^W$ & Neural Network weights\\
        $\Phi_\xi : \Omega_T \rightarrow \R$ & Neural field with weights $\xi$\\
        $P$ & Number of partitions\\
        $\Psi = (\psi^1,\hdots \psi^P)^T$ & Partition of unity \\ 
        $M$ & Number of basis functions \\ 
        $B = (b_1,\hdots , b_M)^T$ &Spanning functions \\ 
        $C \in \R^{P \times M}$ & Coefficient matrix \\ 
        $\ipar^{\Psi,B}_C = \Psi^TCB:$ & POU defined function \\ 
        $\eta$ & Weights of Partition of unity network \\ 
        $\Psi_\eta :\Omega_T \rightarrow \R^P$ & POU parametrized by neural network \\ 
        $\Phi_{(\eta,B)} = f^{\Psi_\eta,B}_C$& POUnet \\
        $\rho > 0$ & Training weight to enforce distribution of partitions\\
        $\tau >0$ & Training weight to promote sparsity of distributions \\
        $\epsilon >0$ & Perturbing term to prevent singularities \\
        $\crt$& Stationary CRT \\ 
        $\crt_D$ & Dynamic CRT \\ 
        
        
    \end{tabular}
\end{table}
